Learning to Reason for Hallucination Span Detection

Large language models (LLMs) often generate hallucinations -- unsupported content that undermines reliability. While most prior works frame hallucination detection as a binary task, many real-world applications require identifying hallucinated spans, which is a multi-step decision making process. This naturally raises the question of whether explicit reasoning can help the complex task of detecting hallucination spans. To answer this question, we first evaluate pretrained models with and without Chain-of-Thought (CoT) reasoning, and show that CoT reasoning has the potential to generate at least one correct answer when sampled multiple times. Motivated by this, we propose RL4HS, a reinforcement learning framework that incentivizes reasoning with a span-level reward function. RL4HS builds on Group Relative Policy Optimization and introduces Class-Aware Policy Optimization to mitigate reward imbalance issue. Experiments on the RAGTruth benchmark (summarization, question answering, data-to-text) show that RL4HS surpasses pretrained reasoning models and supervised fine-tuning, demonstrating the necessity of reinforcement learning with span-level rewards for detecting hallucination spans.

==> Apple/experiments/guided_decoding.tex <==
\begin{table}[ht!]
\begin{adjustbox}{width=\linewidth}
\begin{tabular}{c|ccc|ccc|ccc|ccc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c|}{\textbf{Summarization}} & \multicolumn{3}{c|}{\textbf{QA}} & \multicolumn{3}{c|}{\textbf{Data2Text}} & \multicolumn{3}{c}{\textbf{Avg.}} \\
 & F1 & Precision & Recall & F1 & Precision & Recall & F1 & Precision & Recall & F1 & Precision & Recall \\ \midrule
SFT & 44.1 & 52.2 & 38.2 & 51.3 & 51.3 & 51.4 & 54.8 & 58.8 & 51.5 & 50.1 & 54.1 & 47.0 \\
GRPO w/o COT & 46.5 & 52.2 & \textbf{42.6} & \textbf{59.6} & 54.7 & 65.5 & 53.2 & 52.4 & 56.1 & 53.1 & 53.1 & \textbf{54.7} \\
GRPO w/ COT & \textbf{51.2} & \textbf{68.7} & 40.9 & 55.0 & \textbf{59.6} & 52.1 & \textbf{56.3} & \textbf{66.5} & 48.8 & \textbf{54.2} & \textbf{64.9} & 47.3 \\ \bottomrule
\end{tabular}
% \begin{tabular}{c|ccc|ccc|ccc}
% \toprule
% \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c|}{\textbf{Summarization}} & \multicolumn{3}{c|}{\textbf{Question Answering}} & \multicolumn{3}{c}{\textbf{Data2Text}} \\
%  & F1 & Precision & Recall & F1 & Precision & Recall & F1 & Precision & \multicolumn{1}{c}{Recall} \\ \midrule 
% GRPO w/o COT & 46.5 & 52.2 & 42.6 & \textbf{59.6} & 54.7 & 65.5 & 53.2 & 52.4 & 56.1 \\
% GRPO w/ COT & \textbf{51.2} & \textbf{68.7} & 40.9 & 55.0 & \textbf{59.6} & 52.1 & \textbf{56.3} & \textbf{66.5} & 48.8 \\ \bottomrule
% \end{tabular}


\end{adjustbox}
\caption{Ablation study of GRPO with and without CoT on RAGTruth.  
Both GRPO variants outperform supervised fine-tuning (SFT), confirming the effectiveness of reinforcement learning with span-level rewards.  
GRPO with CoT achieves the best results across tasks, particularly improving precision, showing that reasoning traces enhance policy optimization.}

\label{tab:guided_decode}
\end{table}

==> Apple/experiments/guided_decoding2.tex <==
\begin{wraptable}{r}{0.5\textwidth}
\centering
\small
% \begin{adjustbox}{width=\linewidth}
\begin{tabular}{c|ccc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c}{\textbf{Avg.}} \\
 & F1 & Precision & Recall \\ \midrule
SFT & 50.1 & 54.1 & 47.0 \\
GRPO w/o COT & 53.1 & 53.1 & \textbf{54.7} \\
GRPO w/ COT & \textbf{54.2} & \textbf{64.9} & 47.3 \\ \bottomrule
\end{tabular}
% \begin{tabular}{c|ccc|ccc|ccc}
% \toprule
% \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c|}{\textbf{Summarization}} & \multicolumn{3}{c|}{\textbf{Question Answering}} & \multicolumn{3}{c}{\textbf{Data2Text}} \\
%  & F1 & Precision & Recall & F1 & Precision & Recall & F1 & Precision & \multicolumn{1}{c}{Recall} \\ \midrule 
% GRPO w/o COT & 46.5 & 52.2 & 42.6 & \textbf{59.6} & 54.7 & 65.5 & 53.2 & 52.4 & 56.1 \\
% GRPO w/ COT & \textbf{51.2} & \textbf{68.7} & 40.9 & 55.0 & \textbf{59.6} & 52.1 & \textbf{56.3} & \textbf{66.5} & 48.8 \\ \bottomrule
% \end{tabular}


% \end{adjustbox}
\caption{\textbf{Ablation study of GRPO with and without CoT on RAGTruth.}   
GRPO with CoT achieves the best results across tasks, particularly improving precision, showing that reasoning traces enhance policy optimization.}
\label{tab:guided_decode}
\end{wraptable}


==> Apple/experiments/loss_function_table.tex <==
\begin{table}[ht!]
\begin{adjustbox}{width=\linewidth}

\begin{tabular}{llllllllll}
\toprule
                           & \multicolumn{3}{l}{Summarization} & \multicolumn{3}{l}{Question Answering} & \multicolumn{3}{l}{Data-to-Text} \\ \midrule
                           & F1        & Precision         & Recall         & F1     & Precision     & Recall     & F1       & Precision        & Recall       \\
GRPO with Strict Naive Prompt & 0.532     & 0.562     & 0.506     & 0.487  & 0.479 & 0.498 & 0.520    & 0.690    & 0.417   \\
HS-R1                   & 0.541     & 0.617     & 0.491     & 0.478  & 0.485 & 0.479 & 0.582    & 0.665    & 0.518   \\ \bottomrule
\end{tabular}

\end{adjustbox}
\caption{\textbf{Comparison of HS-R1 variants for hallucination span detection on RAGTruth.} 
We report span F1, precision, and recall across summarization, question answering, and data-to-text. 
HS-R1 with Naive Prompt trains using the naive prompting format, while HS-R1 with Strict Naive Prompt further restricts the output to direct answers with limited length. 
Standard HS-R1 uses our default setup with reasoning-style prompting. 
Results show that although stricter prompting improves recall in some cases, reasoning-based HS-R1 achieves more balanced performance overall.
}
\label{tab:loss}
\end{table}

==> Apple/experiments/main-table-response-f1.tex <==
\begin{table}[ht!]
\begin{adjustbox}{width=\linewidth}

\begin{tabular}{ccccccccccc}
\toprule
\textbf{RESPONSE-F1} &  & \multicolumn{3}{c}{\textbf{Summarization}} & \multicolumn{3}{c}{\textbf{Question Answering}} & \multicolumn{3}{c}{\textbf{Data2Text}} \\ \midrule
 &  & F1 & \multicolumn{1}{c}{Precision} & \multicolumn{1}{c}{Recall} & F1 & \multicolumn{1}{c}{Precision} & \multicolumn{1}{c}{Recall} & F1 & \multicolumn{1}{c}{Precision} & \multicolumn{1}{c}{Recall} \\
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Instruction-tuned \\ Model\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Qwen2.5 7B Instruct\\ Naive Prompt\end{tabular} & \multicolumn{1}{l}{0.463} & 0.466 & 0.460 & \multicolumn{1}{l}{0.357} & 0.254 & 0.598 & \multicolumn{1}{l}{0.653} & 0.731 & 0.589 \\
 & \begin{tabular}[c]{@{}c@{}}Qwen2.5 7B Instruct\\ COT\end{tabular} & \multicolumn{1}{l}{0.480} & 0.371 & 0.678 & \multicolumn{1}{l}{0.368} & 0.250 & 0.699 & \multicolumn{1}{l}{0.664} & 0.757 & 0.591 \\ \midrule
\multirow{3}{*}{Reasoning Model} & QwQ-32B COT & 0.619 & \multicolumn{1}{c}{0.504} & \multicolumn{1}{c}{0.830} & 0.533 & \multicolumn{1}{c}{0.425} & \multicolumn{1}{c}{0.716} & 0.587 & \multicolumn{1}{c}{0.822} & \multicolumn{1}{c}{0.457} \\
 & Qwen3-8B COT & 0.631 & \multicolumn{1}{c}{0.539} & \multicolumn{1}{c}{0.760} & 0.516 & \multicolumn{1}{c}{0.371} & \multicolumn{1}{c}{0.845} & 0.550 & \multicolumn{1}{c}{0.767} & \multicolumn{1}{c}{0.429} \\
 & Qwen3-14B COT & 0.595 & \multicolumn{1}{c}{0.452} & \multicolumn{1}{c}{0.870} & 0.491 & \multicolumn{1}{c}{0.340} & \multicolumn{1}{c}{0.884} & 0.715 & \multicolumn{1}{c}{0.762} & \multicolumn{1}{c}{0.673} \\ \midrule
\multirow{4}{*}{Finetuned Model} & SFT-7B & \multicolumn{1}{l}{0.699} & 0.688 & 0.714 & \multicolumn{1}{l}{0.700} & 0.646 & 0.766 & \multicolumn{1}{l}{0.904} & 0.913 & 0.896 \\
 & SFT - 14B & \multicolumn{1}{l}{0.736} & 0.711 & 0.763 & \multicolumn{1}{l}{0.698} & 0.626 & 0.788 & \multicolumn{1}{l}{0.912} & 0.926 & 0.898 \\
 & HS-R1 - 7B & \multicolumn{1}{l}{0.692} & 0.713 & 0.675 & \multicolumn{1}{l}{0.728} & 0.685 & 0.779 & \multicolumn{1}{l}{0.899} & 0.908 & 0.889 \\
 & HS-R1 - 14B &  & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} &  & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} &  & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} \\ \bottomrule
\end{tabular}

\end{adjustbox}
\caption{\textbf{Response-level hallucination detection results on RAGTruth.} 
We report F1, precision, and recall across summarization, question answering, and data-to-text. 
Naive and CoT are pretrained prompting baselines, while SFT is supervised fine-tuning. 
HS-R1 uses reinforcement learning with span rewards, and adds dynamic sampling. 
CAPO (ours) applies class-aware sampling. 
Best scores are in bold.
}
\label{tab:main-response-f1}
\end{table}

==> Apple/experiments/main-table-std.tex <==
\begin{table}[h]
\caption{\textbf{Span-level hallucination detection results (STD) on RAGTruth.} 
}
\centering
\begin{adjustbox}{width=\linewidth}
\begin{tabular}{cccccccccc}
\toprule
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Model}}} & \multicolumn{3}{c|}{\textbf{Summarization}} & \multicolumn{3}{c|}{\textbf{Question Answering}} & \multicolumn{3}{c}{\textbf{Data2Text}} \\
\multicolumn{1}{c|}{} & F1 & Precision & \multicolumn{1}{c|}{Recall} & F1 & Precision & \multicolumn{1}{c|}{Recall} & F1 & Precision & Recall \\ \midrule
\multicolumn{1}{l}{\textit{\textbf{Proprietary models}}} &  &  &  &  &  &  &  &  &  \\ \midrule
\multicolumn{1}{c|}{GPT-4o-mini w/ COT} & 1.5 & 1.9 & \multicolumn{1}{c|}{1.5} & 0.6 & 0.7 & \multicolumn{1}{c|}{0.8} & 1.9 & 2.1 & 1.9 \\
\multicolumn{1}{c|}{GPT-5-mini w/ COT} & 1.0 & 0.9 & \multicolumn{1}{c|}{{1.4}} & 0.5 & 0.4 & \multicolumn{1}{c|}{0.9} & 1.5 & 1.1 & \textbf{2.5} \\
\multicolumn{1}{c|}{GPT-5 w/ COT} & 0.5 & 0.4 & \multicolumn{1}{c|}{1.2} & 0.4 & 0.4 & \multicolumn{1}{c|}{1.1} & 0.9 & 0.6 & 1.7 \\
\multicolumn{1}{c|}{O3 w/ COT} & 0.8 & 0.8 & \multicolumn{1}{c|}{1.4} & 0.5 & 0.5 & \multicolumn{1}{c|}{0.8} & 2.1 & 1.5 & 3.3 \\ \midrule
\multicolumn{1}{l}{\textit{\textbf{Non-Reasoning models}}} &  &  &  &  &  &  &  &  &  \\ \midrule
\multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Qwen2.5-7B-Instruct\\ w/o COT\end{tabular}} & 1.7 & 2.5 & \multicolumn{1}{c|}{1.4} & 1.1 & 1.3 & \multicolumn{1}{c|}{0.9} & 1.1 & 1.3 & 0.9 \\
\multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Qwen2.5-7B-Instruct\\ w/ COT\end{tabular}} & 2.0 & 2.7 & \multicolumn{1}{c|}{1.8} & 1.1 & 1.3 & \multicolumn{1}{c|}{0.9} & 1.0 & 2.6 & 0.7 \\
\multicolumn{1}{c|}{Qwen2.5-14B-Instruct w/o COT} & 1.3 & 1.3 & \multicolumn{1}{c|}{1.5} & 0.7 & 0.7 & \multicolumn{1}{c|}{0.9} & 0.6 & 0.6 & 0.7 \\
\multicolumn{1}{c|}{Qwen2.5-14B-Instruct w/ COT} & 2.3 & 2.8 & \multicolumn{1}{c|}{2.2} & 1.8 & 3.0 & \multicolumn{1}{c|}{1.4} & 1.3 & 1.9 & 1.1 \\ \midrule
\multicolumn{1}{l}{\textit{\textbf{Reasoning models}}} &  &  &  &  &  &  &  &  &  \\ \midrule
\multicolumn{1}{c|}{QwQ-32B} & 1.9 & 3.8 & \multicolumn{1}{c|}{1.3} & 1.4 & 4.0 & \multicolumn{1}{c|}{0.9} & 1.0 & 2.6 & 0.6 \\
\multicolumn{1}{c|}{Qwen3-8B} & 2.1 & 2.4 & \multicolumn{1}{c|}{2.2} & 2.2 & 1.8 & \multicolumn{1}{c|}{2.6} & 1.4 & 2.7 & 1.0 \\
\multicolumn{1}{c|}{Qwen3-14B} & 1.8 & 2.0 & \multicolumn{1}{c|}{1.8} & 1.9 & 1.8 & \multicolumn{1}{c|}{2.1} & 1.1 & 1.2 & 1.3 \\ \midrule
\multicolumn{1}{l}{\textit{\textbf{Finetuned models}}} &  &  &  &  &  &  &  &  &  \\ \midrule
\multicolumn{1}{c|}{SFT-7B} & 1.4 & 2.8 & \multicolumn{1}{c|}{0.6} & 0.3 & 1.6 & \multicolumn{1}{c|}{1.2} & 0.4 & 2.4 & 2.4 \\
\multicolumn{1}{c|}{SFT-14B} & 1.2 & 3.2 & \multicolumn{1}{c|}{0.5} & 0.7 & 1.0 & \multicolumn{1}{c|}{0.5} & 0.6 & 1.8 & 0.5 \\
\multicolumn{1}{c|}{Multi-View Attention-7B} & N/A & N/A & \multicolumn{1}{c|}{N/A} & N/A & N/A & \multicolumn{1}{c|}{N/A} & N/A & N/A & N/A \\ \midrule
\multicolumn{1}{l}{\textit{\textbf{Ours: \ours}}} &  &  &  &  &  &  &  &  &  \\ \midrule
\multicolumn{1}{c|}{\ours-GRPO-7B} & 1.0 & 2.2 & \multicolumn{1}{c|}{1.3} & 2.4 & 7.5 & \multicolumn{1}{c|}{4.5} & 0.5 & 0.5 & 0.4 \\
\multicolumn{1}{c|}{\ours-7B} & 0.5 & {0.5} & \multicolumn{1}{c|}{0.4} & {4.4} & {4.8} & \multicolumn{1}{c|}{7.3} & 0.3 & 1.5 & 1.6 \\
\multicolumn{1}{c|}{\ours-14B} & {1.1} & 1.0 & \multicolumn{1}{c|}{1.9} & 1.1 & 1.0 & \multicolumn{1}{c|}{1.9} & {0.7} & {1.7} & 2.4 \\ \bottomrule
\end{tabular}


% \begin{tabular}{cccccccccc}
% \toprule
% \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Model}}} & \multicolumn{3}{c|}{\textbf{Summarization}} & \multicolumn{3}{c|}{\textbf{Question Answering}} & \multicolumn{3}{c}{\textbf{Data-to-Text}} \\
% \multicolumn{1}{c|}{} & F1 & Precision & \multicolumn{1}{c|}{Recall} & F1 & Precision & \multicolumn{1}{c|}{Recall} & F1 & Precision & Recall \\ \midrule
% \multicolumn{10}{l}{\textit{\textbf{Proprietary models}}} \\ \midrule
% \multicolumn{1}{c|}{GPT-4-mini w/ COT} & 38.4 & 43.4 & \multicolumn{1}{c|}{34.4} & 27.3 & 33.7 & \multicolumn{1}{c|}{23.0} & 33.7 & 34.2 & 33.2 \\
% \multicolumn{1}{c|}{GPT-5-mini w/ COT} & 43.9 & 33.0 & \multicolumn{1}{c|}{\textbf{65.5}} & 47.2 & 37.9 & \multicolumn{1}{c|}{62.7} & 42.5 & 29.8 & \textbf{74.7} \\ \midrule
% \multicolumn{10}{l}{\textit{\textbf{Non-Reasoning models}}} \\ \midrule
% \multicolumn{1}{c|}{Qwen2.5-7B-Instruct w/o COT} & 19.3 & 28.9 & \multicolumn{1}{c|}{14.5} & 14.7 & 19.2 & \multicolumn{1}{c|}{11.9} & 14.0 & 22.3 & 10.2 \\
% \multicolumn{1}{c|}{Qwen2.5-7B-Instruct w/ COT} & 21.0 & 27.4 & \multicolumn{1}{c|}{17.1} & 14.5 & 18.8 & \multicolumn{1}{c|}{11.7} & 13.0 & 32.5 & 8.2 \\ \midrule
% \multicolumn{10}{l}{\textit{\textbf{Reasoning models}}} \\ \midrule
% \multicolumn{1}{c|}{QwQ-32B w/ COT} & 19.4 & 50.6 & \multicolumn{1}{c|}{12.0} & 12.9 & 48.5 & \multicolumn{1}{c|}{7.5} & 13.5 & 60.7 & 7.6 \\
% \multicolumn{1}{c|}{Qwen3-8B w/ COT} & 34.7 & 42.2 & \multicolumn{1}{c|}{29.5} & 30.5 & 32.0 & \multicolumn{1}{c|}{29.1} & 20.3 & 45.2 & 13.1 \\
% \multicolumn{1}{c|}{Qwen3-14B w/ COT} & 35.8 & 36.9 & \multicolumn{1}{c|}{34.9} & 30.6 & 30.7 & \multicolumn{1}{c|}{30.6} & 34.8 & 40.9 & 30.4 \\ \midrule
% \multicolumn{10}{l}{\textit{\textbf{Finetuned models}}} \\ \midrule
% \multicolumn{1}{c|}{SFT-7B} & 44.1 & 52.2 & \multicolumn{1}{c|}{38.2} & 51.3 & 51.3 & \multicolumn{1}{c|}{51.4} & 54.8 & 58.8 & 51.5 \\
% \multicolumn{1}{c|}{SFT-14B} & 52.7 & 57.6 & \multicolumn{1}{c|}{48.7} & 53.9 & 53.1 & \multicolumn{1}{c|}{54.8} & 59.6 & 61.6 & 57.8 \\
% \multicolumn{1}{c|}{Lookback Lens-7B} & 0.0 & 0.0 & \multicolumn{1}{c|}{0.0} & 10.0 & 5.6 & \multicolumn{1}{c|}{46.6} & 0.0 & 50.0 & 0.0 \\
% \multicolumn{1}{c|}{Multi-View Attention-7B} & 41.5 & 49.6 & \multicolumn{1}{c|}{35.7} & 50.6 & 38.5 & \multicolumn{1}{c|}{\textbf{73.7}} & 55.2 & 53.5 & 57.1 \\ \midrule
% \multicolumn{10}{l}{\textit{\textbf{Ours: \ours}}} \\ \midrule
% \multicolumn{1}{c|}{\ours-7B} & 50.9 & \textbf{64.4} & \multicolumn{1}{c|}{42.3} & \textbf{56.4} & \textbf{57.1} & \multicolumn{1}{c|}{56.5} & 60.4 & 67.1 & 54.9 \\
% \multicolumn{1}{c|}{\ours-14B} & \textbf{57.6} & 64.2 & \multicolumn{1}{c|}{52.3} & 54.8 & 52.5 & \multicolumn{1}{c|}{57.3} & \textbf{62.6} & \textbf{67.2} & 58.7 \\ \bottomrule
% \end{tabular}

\end{adjustbox}
% \caption{\textbf{Span-level hallucination detection results (STD) on RAGTruth.} 
% }
\label{tab:main_std}
\end{table}

==> Apple/experiments/ood.tex <==
\begin{table}[ht!]
\begin{adjustbox}{width=\linewidth}
\begin{tabular}{c|ccc|ccc|ccc|ccc}
\toprule
\textbf{Source} &
  \multicolumn{3}{c|}{\textbf{QA + Data2Text}} &
  \multicolumn{3}{c|}{\textbf{Summarization + Data2Text}} &
  \multicolumn{3}{c|}{\textbf{QA+Summarization}} &
  \multicolumn{3}{c}{\multirow{2}{*}{\textbf{Avg.}}} \\
\textbf{Target} &
  \multicolumn{3}{c|}{\textbf{Summarization}} &
  \multicolumn{3}{c|}{\textbf{QA}} &
  \multicolumn{3}{c|}{\textbf{Data2Text}} &
  \multicolumn{3}{c}{} \\
\textbf{Method} &
  F1 &
  Precision &
  Recall &
  F1 &
  Precision &
  Recall &
  F1 &
  Precision &
  Recall &
  F1 &
  Precision &
  Recall \\ \midrule
SFT-7B &
  42.9 &
  55.5 &
  \textbf{35.1} &
  29.2 &
  36.2 &
  \textbf{24.6} &
  25.6 &
  20.8 &
  33.6 &
  32.6 &
  37.5 &
  \textbf{31.1} \\
HS-R1-7B &
  \textbf{46.1} &
  \textbf{73.9} &
  33.6 &
  27.3 &
  \textbf{48.5} &
  19.4 &
  \textbf{38.3} &
  \textbf{39.2} &
  \textbf{38.1} &
  \textbf{37.2} &
  \textbf{53.9} &
  30.4 \\ \bottomrule
\end{tabular}

% \begin{tabular}{c|ccc|ccc|ccc}
% \toprule
% \textbf{Source Task} &
%   \multicolumn{3}{c|}{\textbf{QA + Data2Text}} &
%   \multicolumn{3}{c|}{\textbf{Summarization + Data2Text}} &
%   \multicolumn{3}{c}{\textbf{QA+Summarization}} \\
% \textbf{Target Task} &
%   \multicolumn{3}{c|}{\textbf{Summarization}} &
%   \multicolumn{3}{c|}{\textbf{QA}} &
%   \multicolumn{3}{c}{\textbf{Data2Text}} \\
% \textbf{Method} &
%   F1 &
%   Precision &
%   Recall &
%   F1 &
%   Precision &
%   Recall &
%   F1 &
%   Precision &
%   Recall \\ \midrule
% SFT &
%   42.9 &
%   55.5 &
%   \textbf{35.1} &
%   \textbf{29.2} &
%   36.2 &
%   \textbf{24.6} &
%   25.6 &
%   20.8 &
%   33.6 \\
% HS-R1 &
%   \textbf{46.1} &
%   \textbf{73.9} &
%   33.6 &
%   27.3 &
%   \textbf{48.5} &
%   19.4 &
%   \textbf{38.3} &
%   \textbf{39.2} &
%   \textbf{38.1} \\ \bottomrule
% \end{tabular}

\end{adjustbox}
\caption{\textbf{Leave-one-out evaluation on RAGTruth.} Models are trained on two tasks and evaluated on the held-out target task. HS-R1 consistently outperforms SFT in out-of-distribution (OOD) settings, showing more balanced precision and recall. Together with results in Table~\ref{tab:main}, this highlights that pretrained reasoning models alone are insufficient, and hallucination-specific fine-tuning with span-level rewards is necessary for robustness.}

\label{tab:ood}
\end{table}

==> Apple/sections/4-Reasoning_for_Hallucination_Detection.tex <==
\section{Potential of CoT Reasoning - Motivation for RL}
\label{sec:cot}
A central question in our research is whether explicit reasoning is beneficial for identifying hallucination spans. As a preliminary experiment, we evaluated \texttt{Qwen2.5-7B}~\footnote{We use the instruct version.} and \texttt{Qwen3-8B} models with and without CoT reasoning on data from three CNLG tasks, namely summarization, question answering and data-to-text using the RAGTruth dataset~\citep{wu2023ragtruth}. In CoT reasoning mode, the model is encouraged to first reason about the factual consistency between the input context and the generated output, and then predict hallucinated spans. In the non-reasoning mode, the model is asked to directly predict hallucination spans without generating any intermediate content. Each model is run $K$ times and the best prediction is selected based on span-F1. We repeat this experiment for different values of $K$ and show the corresponding Span-F1@K results in Figure~\ref{fig:f1@k}.

At $K=1$, CoT reasoning provides no gains for \texttt{Qwen2.5-7B} and limited gains for \texttt{Qwen3-8B}. However, as $K$ increases, the gap in terms of Span-F1@K increases significantly demonstrating the potential of CoT reasoning to generate at least one accurate prediction when sampled multiple times. These results provide clear motivation to use reinforcement learning for bringing the reasoning capacity of LLMs related to hallucination span detection to the forefront.

We also conducted this experiment with \texttt{Qwen3-14B} model and observed a similar behavior. See Appendix for details.\TODO{Ravi: Add link to the appendix section}
\input{Apple/experiments/f1@k}

% These models achieve stronger hallucination detection than standard instruction-tuned baselines, indicating that general-purpose reasoning ability can partially transfer to this task. 
% Nonetheless, the performance gap between naive prompting and CoT prompting remains narrow, showing that reasoning skills acquired from unrelated tasks are not directly sufficient for robust hallucination detection.

% At $K=1$, CoT provides little or no advantage over naive prompting, consistent with prior findings. 
% However, for larger $K$, the trend reverses: CoT yields consistent gains, and for $K \geq 8$ the improvement becomes substantial. 
% This suggests that while CoT does not guarantee better performance in single samples, it increases the likelihood of producing at least one accurate detection among multiple generations.

% Prior work \cite{luo2023chatgptfactualinconsistencyevaluator, dhuliawala-etal-2024-chain, cheng2025chainofthoughtpromptingobscureshallucination} has raised doubts that chain-of-thought (CoT) prompting did not lead to consistent gains in factuality evaluation.  

% This raises the concern that CoT may produce superficial reasoning traces without improving actual detection performance.
% To revisit this question, we design below F1@K experiments:
% \subsection{Prompt Design}
% \begin{itemize}[leftmargin=*]
    % \item \textbf{No Chain-of-thought (CoT) prompting:} the model is directly asked to output hallucination spans without providing intermediate reasoning steps.
    % \item\textbf{Chain-of-thought (CoT) prompting:} the model is encouraged to first reason about the factual consistency between the source document and the generated output, and then mark hallucinated spans.
% \end{itemize}

% \paragraph{F1@K}
% \label{sec:f1_k}– 
% In addition to single-response evaluation, we also report F1@K, which measures performance when the model is allowed to generate $K$ candidate outputs via sampling. 
% Let $\hat{S}^{(1)}, \hat{S}^{(2)}, \ldots, \hat{S}^{(K)}$ denote the predicted hallucination span sets from $K$ sampled responses. 
% For each candidate $\hat{S}^{(k)}$, we compute its span-level F1 score against the gold set $S$. 
% F1@K is then defined as
% \[
% \text{F1@K} = \max_{1 \leq k \leq K} \text{F1}(\hat{S}^{(k)}, S),
% \]
% which reflects the best span-level performance achievable among $K$ samples, analogous to Pass@K in mathematical tasks.

% \subsection{F1@K Experiments}
% Figure~\ref{fig:f1@k} reports span-level F1 across $K$ sampled responses. 
% At $K=1$, CoT provides little or no advantage over naive prompting, consistent with prior findings. 
% However, for larger $K$, the trend reverses: CoT yields consistent gains, and for $K \geq 8$ the improvement becomes substantial. 
% This suggests that while CoT does not guarantee better performance in single samples, it increases the likelihood of producing at least one accurate detection among multiple generations.
% \input{Apple/experiments/f1@k}
% \subsection{Pretrained Reasoning Models}
% We also evaluate pretrained reasoning models such as Qwen3-8B and Qwen3-14B. 
% These models achieve stronger hallucination detection than standard instruction-tuned baselines, indicating that general-purpose reasoning ability can partially transfer to this task. 
% Nonetheless, the performance gap between naive prompting and CoT prompting remains narrow, showing that reasoning skills acquired from unrelated tasks are not directly sufficient for robust hallucination detection.



% \subsection{F1@K Experiments}
% We evaluate both prompting strategies under the F1@K setup introduced in Section~\ref{sec:f1_k}, and the results are shown in Figure~\ref{fig:f1@k}. 
% Consistent with prior findings, we observe that at $K=1$ (single response), CoT does not yield clear improvements over naive prompting, and sometimes performs comparably or worse.  
% However, as $K$ increases, a different trend emerges: when the model is allowed to sample multiple responses, CoT substantially improves F1@K.  
% \input{Apple/experiments/f1@k}
% In particular, for $K \geq 8$, CoT outperforms naive prompting by a large margin.  
% This suggests that while CoT reasoning may not guarantee better performance in a single sample, it increases the probability of generating at least one high-quality reasoning trace among multiple samples.


% \begin{tcolorbox}[
%   colback=white,      % white background
%   colframe=AppleBlack,     % black frame
%   coltitle=white,     % black title text
%   title=\textbf{Takeaway 1}
% ]
% Reasoning improves hallucination detection only when combined with multi-sample evaluation (F1@K, $K \geq 8$). 
% Pretrained reasoning models also help, but the small gap between naive and CoT prompting indicates that general reasoning ability alone is not enough for precise hallucination span detection.
% \end{tcolorbox}

==> Apple/sections/6.4_patch_1.tex <==
\subsection{\textbf{Q4: }What is the role of CoT in GRPO training?}
\input{Apple/experiments/guided_decoding}

In Section~\ref{sec:cot}, we showed that chain-of-thought (CoT) prompting alone does not substantially improve hallucination detection in zero-shot settings. A natural question is whether CoT remains useful once the model is fine-tuned with span-level rewards. To answer this, we compare GRPO training with and without CoT guidance (Table~\ref{tab:guided_decode}).

\paragraph{GRPO improves over SFT.} Both GRPO variants outperform supervised fine-tuning, confirming that reinforcement learning with span-level rewards effectively incentivizes hallucination detection.

\paragraph{CoT further enhances GRPO.} GRPO with CoT consistently achieves the strongest performance across tasks. For example, on Summarization it improves span F1 from 46.5 (GRPO w/o CoT) to 51.2, largely driven by a substantial precision gain (68.7 vs.\ 52.2). On QA, CoT maintains comparable precision while improving balance between precision and recall. On Data-to-Text, CoT again boosts both F1 and precision. Overall, GRPO with CoT achieves the best average F1 (54.2) and precision (64.9), showing that reasoning traces provide valuable intermediate structure for policy optimization.

==> Apple/sections/6.4_patch_2.tex <==
\subsection{\textbf{Q4: }What is the role of CoT in GRPO training?}
\input{Apple/experiments/guided_decoding2}
In Section~\ref{sec:cot}, we showed that chain-of-thought (CoT) prompting alone does not  
substantially improve hallucination detection in zero-shot settings. A natural question is whether CoT remains useful once the model is fine-tuned with span-level rewards. To answer this, we compare GRPO training with and without CoT guidance (Table~\ref{tab:guided_decode}). 
Table~\ref{tab:guided_decode} compares GRPO training with and without chain-of-thought (CoT) guidance. Both GRPO variants outperform supervised fine-tuning (SFT), confirming that reinforcement learning with span-level rewards is more effective. However, adding CoT further enhances performance. Specifically, GRPO with CoT achieves the best average F1 (54.2) and precision (64.9), showing that reasoning traces provide useful intermediate structure for policy optimization. Without CoT, GRPO yields slightly higher recall (54.7), but the tradeoff is less favorable. Overall, CoT-guided GRPO offers the strongest balance, demonstrating that reasoning signals meaningfully improve training beyond direct span supervision.
% \paragraph{GRPO improves over SFT.} Both GRPO variants outperform supervised fine-tuning, confirming that reinforcement learning with span-level rewards 
% effectively incentivizes hallucination detection.
% \paragraph{CoT further enhances GRPO.} GRPO with CoT consistently achieves the strongest performance across tasks. For example, on Summarization it improves span F1 from 46.5 (GRPO w/o CoT) to 51.2, largely driven by a substantial precision gain (68.7 vs.\ 52.2). On QA, CoT maintains comparable precision while improving balance between precision and recall. On Data-to-Text, CoT again boosts both F1 and precision. Overall, GRPO with CoT achieves the best average F1 (54.2) and precision (64.9), showing that reasoning traces provide valuable intermediate structure for policy optimization.

